Single-view Neural Radiance Fields with Depth Teacher

Neural Radiance Fields (NeRF) have been proposed for photorealistic novel view rendering. However, it requires many different views of one scene for training. Moreover, it has poor generalizations to new scenes and requires retraining or fine-tuning on each scene. In this paper, we develop a new NeRF model for novel view synthesis using only a single image as input. We propose to combine the (coarse) planar rendering and the (fine) volume rendering to achieve higher rendering quality and better generalizations. We also design a depth teacher net that predicts dense pseudo depth maps to supervise the joint rendering mechanism and boost the learning of consistent 3D geometry. We evaluate our method on three challenging datasets. It outperforms state-of-the-art single-view NeRFs by achieving 5$\sim$20\% improvements in PSNR and reducing 20$\sim$50\% of the errors in the depth rendering. It also shows excellent generalization abilities to unseen data without the need to fine-tune on each new scene.

==> image/comparison.tex <==
\begin{figure}[H]
\centering
\subfigcapskip=5pt
\subfigbottomskip=2pt
\subfigure[SrcView]{
\begin{minipage}[t]{0.15\linewidth}
\centering
\includegraphics[width=1in]{figure/compare/fern_IMG_4031.JPG}
\quad
\includegraphics[width=1in]{figure/compare/flower_IMG_2966.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fortress_IMG_1809.JPG}
%\caption{fig2}
\end{minipage}%
}%
\subfigure[GT]{
\begin{minipage}[t]{0.15\linewidth}
\centering
\includegraphics[width=1in]{figure/compare/fern_IMG_4044.JPG}
\quad
\includegraphics[width=1in]{figure/compare/flower_IMG_2967.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fortress_IMG_1810.JPG}
%\caption{fig2}
\end{minipage}%
}%
\subfigure[PixelSynth]{
\begin{minipage}[t]{0.15\linewidth}
\centering
\includegraphics[width=1in]{figure/compare/fern_IMG_4044.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fern_IMG_4044.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fern_IMG_4044.JPG}
%\caption{fig2}
\end{minipage}%
}%
\subfigure[pixelNeRF]{
\begin{minipage}[t]{0.15\linewidth}
\centering
\includegraphics[width=1in]{figure/compare/fern_pixelnerf_IMG_4044.JPG}
\quad
\includegraphics[width=1in]{figure/compare/flower_pixelnerf_IMG_2967.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fortress_pixelnerf_IMG_1810.JPG}
%\caption{fig2}
\end{minipage}
}%
\subfigure[MINE]{
\begin{minipage}[t]{0.15\linewidth}
\centering
\includegraphics[width=1in]{figure/compare/fern_MINE_IMG_4044.JPG}
\quad
\includegraphics[width=1in]{figure/compare/flower_MINE_IMG_2967.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fortress_MINE_IMG_1810.JPG}
%\caption{fig1}
\end{minipage}%
}%
\subfigure[Ours]{
\begin{minipage}[t]{0.15\linewidth}
\centering
\includegraphics[width=1in]{figure/compare/fern_IMG_4044.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fern_IMG_4044.JPG}
\quad
\includegraphics[width=1in]{figure/compare/fern_IMG_4044.JPG}
%\caption{fig2}
\end{minipage}
}%
% \vspace{1mm}
\caption{Foreground vehicles}
% \vspace{2mm}
\end{figure}

==> image/depth_map.tex <==
\begin{figure*}[t!] \centering
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{lcccc}
     \raisebox{3\totalheight}{w/ DPT} &  {\includegraphics[width=0.2\textwidth]{figure/null.png}} &  {\includegraphics[width=0.2\textwidth]{figure/null.png}} &  {\includegraphics[width=0.2\textwidth]{figure/null.png}} & {\includegraphics[width=0.2\textwidth]{figure/null.png}} \tabularnewline
     
     \raisebox{3\totalheight}{w/o DPT} &  {\includegraphics[width=0.2\textwidth]{figure/null.png}} &  {\includegraphics[width=0.2\textwidth]{figure/null.png}} &  {\includegraphics[width=0.2\textwidth]{figure/null.png}} & {\includegraphics[width=0.2\textwidth]{figure/null.png}} \tabularnewline
     
\end{tabular}
    % \vspace{1pt}
    \caption{depth map} 
    \label{fig:depth_map}
    % \vspace{-4pt}
\end{figure*}

==> image/intro_compare.tex <==
\begin{figure}[t]
\setlength{\abovecaptionskip}{7pt}
\setlength{\belowcaptionskip}{0pt}
	\centering
% 	\subfigure[MINE (PSNR:14.9)]{  % for AAAI
	\subfloat[MINE (PSNR:14.9)]{
%			\centering
			\includegraphics[width=0.23\textwidth]{figure/intro/DJI_20200223_163206_598_0_MINE.png}
%			\label{subfig:pixelnerf}
	}\subfloat[MINE (depth)]{
%			\centering
			\includegraphics[width=0.23\textwidth]{figure/intro/MINE_disp.png}
%			\label{subfig:mpi}
	}
	\\[-3mm]
	\subfloat[Ours (PSNR:17.0)]{
%			\centering
			\includegraphics[width=0.23\textwidth]{figure/intro/DJI_20200223_163206_598_0_ours.png} 
	}\subfloat[Ours (depth)]{
%			\centering
			\includegraphics[width=0.23\textwidth]{figure/intro/ours_disp.png}
	}
	\caption{Comparison with state-of-the-art methods. (a-b) RGB and depth rendering results of  \cite{Li_2021_ICCV2}. It produces many blurs and floats in the occluded regions and at the object/depth edges. 
	(c-d) Our method employs a joint rendering mechanism that preserves more image details and predicts sharp depth edges.}
	\label{fig:performance_illustration}
\end{figure}

==> image/kitti_compare_rgb.tex <==
\begin{figure*}[t!] \centering
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{lccc}
     \raisebox{2\totalheight}{Input} &  
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} 
     \tabularnewline
     
     \raisebox{2\totalheight}{Target GT\,\,\,} &  
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} &
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} 
     \tabularnewline
     
     \raisebox{2\totalheight}{MPI} &  
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} 
     \tabularnewline
     
     \raisebox{2\totalheight}{MINE} &  
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}}
     \tabularnewline
     
     \raisebox{2\totalheight}{Ours} &  
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}} & 
     {\includegraphics[width=0.29\textwidth]{figure/null.png}}
\end{tabular}
    % \vspace{1pt}
    \caption{Qualitative comparison on KITTI. Note that these examples are not cherry-picked, they are the same images used in \cite{Tucker_2020_CVPR}.} 
    \label{fig_kitti_vis}
    % \vspace{-4pt}
\end{figure*} 

==> image/llff_compare.tex <==
\begin{figure*}[th!] \centering
\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{-8pt}
\small
\setlength{\tabcolsep}{1pt}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ccccc}
      MPI & MINE & PixelNeRF & Ours &GT 
     \\
%     \includegraphics[width=0.15\textwidth]{figure/llff compare/src/IMG_1809_src0.png} &
 \includegraphics[width=0.15\textwidth]{figure/llff compare/MPI/IMG_1809_0.png} & 
     \includegraphics[width=0.15\textwidth]{figure/llff compare/MINE/IMG_1809_0.png}& 
     \includegraphics[width=0.15\textwidth]{figure/llff compare/pixelnerf/fortress.png}& 
     \includegraphics[width=0.15\textwidth]{figure/llff compare/ours/IMG_1809_0.png}  &
     \includegraphics[width=0.15\textwidth]{figure/llff compare/gt/IMG_1809.png} 
     \\
     
\end{tabular}
}
    \caption{Comparison on NeRF-LLFF scenes. Models are trained on the LLFF training set and evaluated on the LLFF test set.  Compared with  MPI, MINE and PixelNeRF, our DT-NeRF produces clear scenes with more details and fewer blurs or floats.} 
    % \vspace{-8pt}
    \label{fig:llff_rgb}
\end{figure*}

==> image/llff_compare2.tex <==
\begin{figure*}[th!] \centering
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{lcccc}
     \raisebox{2\totalheight}{Plane} &  {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c/DJI_20200226_143918_576_0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c/DJI_20200226_143918_576_disp0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c/IMG_4044_0.JPG}} & 
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c/IMG_4044_disp0.JPG}} \tabularnewline
     
     \raisebox{2\totalheight}{Plane+inpaint} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c_inpaint/DJI_20200226_143918_576_0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c_inpaint/DJI_20200226_143918_576_disp0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c_inpaint/IMG_4044_0.JPG}} & 
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/c_inpaint/IMG_4044_disp0.JPG}} \tabularnewline
     
     \raisebox{2\totalheight}{Plane+Volume($N = 16$)} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f/DJI_20200226_143918_576_0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f/DJI_20200226_143918_576_disp0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f/IMG_4044_0.JPG}} & 
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f/IMG_4044_disp0.JPG}}\tabularnewline
     
     \raisebox{2\totalheight}{Plane+Volume($N = 16$)+inpaint} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f_inpaint/DJI_20200226_143918_576_0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f_inpaint/DJI_20200226_143918_576_disp0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f_inpaint/IMG_4044_0.JPG}}& 
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/f_inpaint/IMG_4044_disp0.JPG}}\tabularnewline
     
     \raisebox{2\totalheight}{Volume($N = 16$)} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly/DJI_20200226_143918_576_0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly/DJI_20200226_143918_576_disp0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly/IMG_4044_0.JPG}}&
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly/IMG_4044_disp0.JPG}}\tabularnewline
     
     \raisebox{2\totalheight}{Volume($N = 16$)+inpaint} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly_inpaint/DJI_20200226_143918_576_0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly_inpaint/DJI_20200226_143918_576_disp0.JPG}} &  
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly_inpaint/IMG_4044_0.JPG}}&
     {\includegraphics[width=0.2\textwidth]{figure/llff compare2/fonly_inpaint/IMG_4044_disp0.JPG}}
\end{tabular}
    % \vspace{1pt}
    \caption{importance sampling} 
    \label{fig_kitti_vis}
    % \vspace{-4pt}
\end{figure*}

==> image/llff_is.tex <==
\begin{figure}[t]
\centering
\setlength{\abovecaptionskip}{2pt}
\setlength{\belowcaptionskip}{-8pt}
%\setlength{\tabcolsep}{0pt}
%\renewcommand{\arraystretch}{0.0}
%\resizebox{\columnwidth}{!}{
\subfigure[Planar rendering]{
\begin{minipage}[b]{0.45\linewidth}
     \includegraphics[width=1\linewidth]{figure/llff is compare/rgb_nois.png}\\
     \includegraphics[width=1\linewidth]{figure/llff is compare/depth_nois.png} 
\end{minipage}
}\hspace{-2mm}
\subfigure[Planar + volume rendering]{
\begin{minipage}[b]{0.45\linewidth}
     \includegraphics[width=1\linewidth]{figure/llff is compare/rgb_is.png}\\
     \includegraphics[width=1\linewidth]{figure/llff is compare/depth_is.png}
\end{minipage}
}
%}
    % \vspace{1pt}
    \caption{Influence of fine volume rendering with importance sampling strategy. The improved areas are highlighted by yellow boxes. Compared with the pure planar rendering, extra fine point samples gives more image details and sharper depth edges.} 
    \label{fig: llff_is}
    % \vspace{-4pt}
\end{figure}

==> image/nyu_depth.tex <==
\begin{figure*}[t!] \centering
\begin{tabular}{ccccc}
     Input & GT & MINE & Ours \\ 
     \includegraphics[width=0.20\textwidth]{figure/nyu/0000_rgb.png} & 
     \includegraphics[width=0.20\textwidth]{figure/nyu/0000_gt.png} & 
     \includegraphics[width=0.20\textwidth]{figure/nyu/0000_MINE.png} &
     \includegraphics[width=0.20\textwidth]{figure/nyu/0000_ours.png} 
     \\
     \includegraphics[width=0.20\textwidth]{figure/nyu/0015_rgb.png} &
     \includegraphics[width=0.20\textwidth]{figure/nyu/0015_gt.png} &
     \includegraphics[width=0.20\textwidth]{figure/nyu/0015_MINE.png} &
     \includegraphics[width=0.20\textwidth]{figure/nyu/0015_ours.png} 
     \\
     \includegraphics[width=0.20\textwidth]{figure/nyu/0003_rgb.png} &
     \includegraphics[width=0.20\textwidth]{figure/nyu/0003_gt.png} &
     \includegraphics[width=0.20\textwidth]{figure/nyu/0003_MINE.png} &
     \includegraphics[width=0.20\textwidth]{figure/nyu/0003_ours.png} \\
\end{tabular}
    \caption{Qualitative comparison for disparity maps.} 
    % \vspace{-8pt}
    \label{fig_depth_vis}
\end{figure*} 

==> table/efficiency.tex <==
% \begin{table*}[th]
% \centering

% \begin{tabular}{c|ccccc}
% \hline 
% Method & SinNeRF & PixelNeRF & MINE($N_c$=32) & MINE($N_c$=64) & Ours \\
% \hline
% Training Speed(h) & 21  & 48  & 1 & 2 & 3.5 \\
% Inference Speed(s/per image) & 4.7 &  10.5  & 0.012 & 0.016 & 0.34 \\
% \hline
% %MPI Preparation Speed(s/per image) & 0 &  0  & 0.077 & 0.138 & 0.125 \\
% Training Memory & 13497  & 6677M  & 17049M & 24945M  & 21387M \\
% Testing Memory & 9107  & 5767M  & 6851M & 12765M & 9521M \\
% \hline
% PSNR & 18.10  & 17.5  & 18.20 & 18.13 & 19.54 \\
% \hline
% \end{tabular}
% \caption{Comparison of efficiency on NeRF-LLFF. The numbers of sampling points of SinNeRF and PixelNeRF are 64 and 96. We set $N_c=32, N_f=16$ in our method and the resolution output is 384 $\times$ 512. MPI preparation speed denotes how fast planar rendering method generates MPI. MPI would only be generated once per scene. }\label{tab:efficiency}
% \end{table*}


\begin{table*}[htbp]
\caption{Comparison of efficiency on NeRF-LLFF. The resolution is 384 $\times$ 512.  The numbers of sampling points of SinNeRF and PixelNeRF are 64 and 96. We set $N_c=32/16, N_f=16$ in our method. %MPI preparation speed denotes how fast planar rendering method generates MPI. MPI would only be generated once per scene.
}
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{c|ccccc}
\hline 
Method & Training Speed(h) & Inference Speed(s) &  Training Memory &Test Memory & PSNR \\ \hline 
SinNeRF & 21  & 4.7 & 13497M  & 9107M  &18.10   \\
PixelNeRF & 48  & 10.5  &  6677M  & 5767M  &17.50 \\ 
MINE($N_c$=32) & 1 & 0.012 &17049M &6851M &18.20  \\
MINE($N_c$=64) & 2 & 0.016 &  24945M  & 12765M & 18.13 \\
Ours ($N_c$=16)& 3 &0.33 &16355M & 6351M& 19.07\\
Ours ($N_c$=32)& 3.5 &0.34 &  21387M & 9521M & 19.54 \\

%MPI Preparation Speed(s/per image) & 0 &  0  & 0.077 & 0.138 & 0.125 \\
\hline 
\end{tabular}}
% \caption{Comparison of efficiency on NeRF-LLFF. The resolution is 384 $\times$ 512.  The numbers of sampling points of SinNeRF and PixelNeRF are 64 and 96. We set $N_c=32/16, N_f=16$ in our method. %MPI preparation speed denotes how fast planar rendering method generates MPI. MPI would only be generated once per scene.
% }
\label{tab:efficiency}
\end{table*}

% Inference Speed(s/per image) & 4.7(s/iter) &  10.5(s/iter)  & 0.012 (mpi:0.077) & inpaint:0.34(w/o inpaint 0.31)(mpi:0.125) \\

%% training speed, test speed 
%%GPU型号，memory， resolution，psnr

%% 近期非nerf方法，3Dphoto。。。

%% ablation study
%% Nc=16,32,64, Nf=16,32
%% MINE,Nc=64,32 bs1
%% pixelnerf, 96

%% DPT nyu, student and teacher novel view depth map

%% backbone，MINE，vit）， inpainting

==> table/importance_sample.tex <==
\begin{table}[t]
% \vspace{1mm}
\small 
\centering
\begin{tabular}{c|ccc}
\hline 
Render method                                            & LPIPS$\downarrow$  & SSIM$\uparrow$  & PSNR$\uparrow$ \\
\hline
Plane & -      & 0.822 & 28.1 \\
Plane+volume($N = 8$)    & -      & 0.851 & 30.1 \\
Plane+volume($N = 16$)     & 0.1603 & 0.868 & 30.2 \\
volume($N = 8$)   & \textbf{0.1559} & \textbf{0.872} & \textbf{30.3} \\
volume($N = 16$)   & \textbf{0.1559} & \textbf{0.872} & \textbf{30.3} \\
\hline
\end{tabular}
\caption{Importance sampling}\label{tab:render_method}
\vspace{-8pt}
\end{table}

==> table/no_nerf.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|ccc}
\hline 
Method     & LPIPS$\downarrow$  & SSIM$\uparrow$  & PSNR$\uparrow$ \\
\hline
3d-photo &       &   &   \\ 
- &      &   &   \\
Ours&   &   &   \\
\hline
\end{tabular}
\caption{not nerf.}\label{tab:nonerf}
\end{table}

==> table/table1.tex <==
\begin{table}[h]

\setlength{\tabcolsep}{7pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\small
\begin{center}
% \begin{tabular}{l |c | c | c |c|c}
\begin{tabular}{l |c | c | c}
\toprule[2pt]


Methods & LPIPS & SSIM & PSNR \%\\
\toprule[1pt]
\hline

PixelSynth~\cite{Rockwell_2021_ICCV} & 1 & 1 & 1 \\\
pixelNeRF~\cite{Yu_2021_CVPR}  &  0.2823 & 0.446 & 17.2 \\\
MINE~\cite{Li_2021_ICCV2} & 0.2750 & 0.433 & 16.7 \\

% \hline
\textbf{ours} & \textbf{1} & 1 & \textbf{1} \\
\toprule[2pt]
\end{tabular}
\end{center}
\caption{Comparison of different linear/efficient Transformer variants on Long Range Arena~\cite{tay2020long}, based on its official configuration. Our SOFT surpasses previous efficient methods on three tasks.
}
\label{tab:lra}
\vspace{-2em}
\end{table}

==> table/table2.tex <==
\begin{table}[!htb]
% \hspace{-2em}
\setlength{\tabcolsep}{11pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \begin{tabular}{l | c | c  }
            \toprule[2pt]
            Methods & Pyramidal?  & Top-1 \%\\
            \toprule[1pt]
            \hline
            DeiT-S~\cite{touvron2020training} & \XSolidBrush  & 79.8\\
            SOFT & \XSolidBrush & 80.1\\
            SOFT & \checkmark & 82.2\\
            \toprule[2pt]
        \end{tabular}
        % \caption{Ablations on bottleneck token sequence length.}
        \label{tab:pyramidal}
    \end{subtable}%
    % \hspace{0.1em}
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \begin{tabular}{l | c | c }
            \toprule[2pt]
            Methods & Overlapped? & Top-1 \%\\
            \toprule[1pt]
            \hline
            PVT~\cite{wang2021pyramid} & \XSolidBrush & 75.1\\
            SOFT & \XSolidBrush & 77.4\\
            SOFT & \checkmark & 79.3\\
            \toprule[2pt]
        \end{tabular}
        \label{tab:overlapping}
        % \caption{Ablations on sampling methods.}
    \end{subtable}
    \caption{(a) Ablations on pyramidal architecture. 
    (b) Ablations on overlapped convolution.}
    \label{tab:pyramidal-overlapping}
\vspace{-2em}
\end{table}
